High-energy spectra of LTT 1445A and GJ 486 reveal flares and activity

The high-energy radiative output, from the X-ray to the ultraviolet, of exoplanet host stars drives photochemical reactions and mass loss in the upper regions of planetary atmospheres. In order to place constraints on the atmospheric properties of the three closest terrestrial exoplanets transiting M dwarfs, we observe the high-energy spectra of the host stars LTT1445A and GJ486 in the X-ray with XMM-Newton and Chandra and in the ultraviolet with HST/COS and STIS. We combine these observations with estimates of extreme ultraviolet flux, reconstructions of the Ly-a lines, and stellar models at optical and infrared wavelengths to produce panchromatic spectra from 1A--20um for each star. While LTT1445Ab, LTT1445Ac, and GJ486b do not possess primordial hydrogen-dominated atmospheres, we calculate that they are able to retain pure CO2 atmospheres if starting with 10, 15, and 50% of Earth's total CO2 budget, respectively, in the presence of their host stars' stellar wind. We use age-activity relationships to place lower limits of 2.2 and 6.6 Gyr on the ages of the host stars LTT1445A and GJ486. Despite both LTT1445A and GJ486 appearing inactive at optical wavelengths, we detect flares at ultraviolet and X-ray wavelengths for both stars. In particular, GJ486 exhibits two flares with absolute energies of 10^29.5 and 10^30.1 erg (equivalent durations of 4357+/-96 and 19724+/-169 s) occurring three hours apart, captured with HST/COS G130M. Based on the timing of the observations, we suggest that these high-energy flares are related and indicative of heightened flaring activity that lasts for a period of days, but our interpretations are limited by sparse time-sampling. Consistent high-energy monitoring is needed to determine the duration and extent of high-energy activity on individual M dwarfs, as well as the population as a whole.

==> extra.tex <==
\begin{comment}
\begin{table*}
\centering
\caption{HST Observations of \LTT\ used in this work\label{tab:obs_LTT1445A}}
\begin{tabular}{c|ccccccccc}
\hline\hline
GO & Visit & Instrument & Orbit & Grating & Central Wavelength & Wavelength Range & Exposure Time & \texttt{FP-POS} \\
&       &       &            &         &(\AA)               & (\AA)            & (s)           & \\
\hline
\multirow{11}{*}{\rotatebox[origin=c]{90}{16722}} & \multirow{4}{*}{01} & \multirow{4}{*}{COS} & 1  &  \multirow{4}{*}{G130M} &  \multirow{4}{*}{1222} &  \multirow{4}{*}{1065--1367} & 2362 & 1 \\
&  &   & 2 & & & & 2700 & 2\\
&  &   & 3 & & & & 1298 & 3 \\
&  &   & 3 & & & & 1297 & 4 \\ 
\cline{2-9}
 & \multirow{6}{*}{52}      & \multirow{6}{*}{COS} & 1 &  \multirow{2}{*}{G230L} & \multirow{2}{*}{2950} & \multirow{2}{*}{1695--3203} &  270  & 2\\
 &      &  & 1    &       &      &            &  270 & 3\\
 \cline{4-9}
 &      &  & 1   & \multirow{4}{*}{G160M} &  \multirow{4}{*}{1533} & \multirow{4}{*}{1339--1710} & 1535  & 1\\
 &      &  & 2    &       &      &            & 2700 & 2 \\
 &      &  & 3    &       &      &            & 1298 & 3\\
 &      &  & 3    &       &      &            & 1297 & 4\\
\cline{2-9}
 & 03 &  STIS  & 1 & G140M & 1222 &    & 2208 &  \\
\hline

\multirow{4}{*}{\rotatebox[origin=c]{90}{16701}} & \multirow{4}{*}{01} & \multirow{4}{*}{STIS} & 1 &  \multirow{2}{*}{G140M} &  \multirow{2}{*}{1222} &  \multirow{2}{*}{} & 1981 &  \\
&  &  & 2 &       &      & & 2507 &  \\
\cline{4-9}
&  &  & 3 & G230L & 2376 & 1581--3143 & 2053 &  \\
\cline{4-9}
&  &  & 3 & G430L & 4300 & 2889--5695 & 60 &  \\
\hline 
\end{tabular}
\tablefoot{Spectra taken with the COS/G130M and COS/G160M gratings were placed at lifetime position four (LP4) on the FUV detector following recommendations by the COS team to mitigate gain sag and extend the detector lifetime. In Visit 02 guide star acquisition failed. This visit was redone and renamed Visit 52.\\
 }
\end{table*}

\begin{table*}
\centering
\caption{HST Observations of \GJ\ used in this work\label{tab:obs_GJ486}}
\begin{tabular}{c|ccccccccc}
\hline\hline
GO & Visit & Instrument & Orbit & Grating & Central Wavelength & Wavelength Range & Exposure Time & \texttt{FP-POS} \\
&       &       &            &         &(\AA)               & (\AA)            & (s)           & \\
\hline
\multirow{11}{*}{\rotatebox[origin=c]{90}{16722}} & \multirow{4}{*}{04} & \multirow{4}{*}{COS} & 1  &  \multirow{4}{*}{G130M} &  \multirow{4}{*}{1222} &  \multirow{4}{*}{1065--1367} & 2337 & 1 \\
&  &   & 2 & & & & 2689 & 2\\
&  &   & 3 & & & & 1292 & 3 \\
&  &   & 3 & & & & 1292 & 4 \\ 
\cline{2-9}
 & \multirow{6}{*}{05}  & \multirow{6}{*}{COS} & 1 & \multirow{2}{*}{G230L} & \multirow{2}{*}{2950} & \multirow{2}{*}{1695--3203} &  276  & 2\\
 &      &  & 1    &       &      &            &  276 & 3\\
 \cline{4-9}
 &      &  & 1   & \multirow{4}{*}{G160M} &  \multirow{4}{*}{1533} & \multirow{4}{*}{1339--1710} & 1480  & 1\\
 &      &  & 2    &       &      &            & 2689 & 2 \\
 &      &  & 3    &       &      &            & 1292 & 3\\
 &      &  & 3    &       &      &            & 1292 & 4\\
\cline{2-9}
 & \multirow{2}{*}{06} &  \multirow{2}{*}{STIS}  & 1 & \multirow{2}{*}{G140M} & \multirow{2}{*}{1222} &    & 2160 &  \\
 &  &  & 2 & & &    & 2723 &  \\
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{16701}} & \multirow{3}{*}{02} & \multirow{3}{*}{STIS} & 2 &  G140M & 1222 &  & 2352 &  \\
\cline{4-9}
&  &  & 3 & G230L & 2376 & 1581--3143 & 2046 &  \\
\cline{4-9}
&  &  & 3 & G430L & 4300 & 2889--5695 & 60 &  \\
\hline 
\end{tabular}
\tablefoot{Spectra taken with the COS/G130M and COS/G160M gratings were placed at lifetime position four (LP4) on the FUV detector following recommendations by the COS team to mitigate gain sag and extend the detector lifetime.\\
 }
\end{table*}
\end{comment}
